Criticality and Saturation in Orthogonal Neural Networks

It has been known for a long time that initializing weight matrices to be orthogonal instead of having i.i.d. Gaussian components can improve training performance. This phenomenon can be analyzed using finite-width corrections, where the infinite-width statistics are supplemented by a power series in $1/\mathrm{width}$. In particular, recent empirical results by Day et al. show that the tensors appearing in this treatment stabilize for large depth, as opposed to the tensors of i.i.d.-initialized networks. In this article, we derive explicit layer-wise recursion relations for the tensors appearing in the finite-width expansion of the network statistics in the case of orthogonal initializations. We also provide an extension of recently-introduced Feynman diagrams for the corresponding recursions in the i.i.d.-case which are valid to all orders in $1/\mathrm{width}$. Finally, we show explicitly that the recursions we derive reproduce the stability of the finite-width tensors which was observed for activation functions with vanishing fixed point. This work therefore provides a theoretical explanation for the stability of nonlinear networks of finite width initialized with orthogonal weights, closing a long-standing gap in the literature. We validate our theoretical results experimentally by showing that numerical solutions of our recursion relations and their analytical large-depth expansions agree excellently with Monte-Carlo estimates from network ensembles.

==> feynman_setup.tex <==
\RequirePackage{tikz}
\usetikzlibrary{shapes, arrows, positioning, decorations, fadings, external}
% \tikzexternalize[prefix=tikz/]
% \tikzsetfigurename{output-figure}
%the two lines above activate externalization!

\RequirePackage{tikz-feynman}
\RequirePackage{feynmp-auto}

\pgfdeclaredecoration{parallel}{initial}{%
  \state{initial}[width=0, next state=main]{\pgfpathmoveto{\pgfpointorigin}}%
  \state{main}[width=\pgfdecoratedinputsegmentlength/100]
  {
    \pgfpathlineto{\pgfpointorigin}
  }%
  \state{final}{}%
}

\tikzfeynmanset{
    color6color1ddntknew/.style={
    dash pattern=on 1pt off 1pt,
    line width=1pt,
    draw=color6,
    opacity=0,
    postaction={
        draw=color1,
        opacity=1,
        decorate,
        decoration={parallel, raise=-0.75pt}
        },
    postaction={
        draw=color6,
        opacity=1,
        decorate,
        decoration={parallel, raise=0.75pt}
        }
    },
    color6color1ddntk2new/.style={
    dash pattern=on 1pt off 1pt,
    line width=1pt,
    draw=color6,
    opacity=0,
    postaction={
        draw=color6,
        opacity=1,
        decorate,
        decoration={parallel, raise=-0.75pt}
        },
    postaction={
        draw=color1,
        opacity=1,
        decorate,
        decoration={parallel, raise=0.75pt}
        }
    },
    color6color2ddntknew/.style={
    dash pattern=on 1pt off 1pt,
    line width=1pt,
    draw=color6,
    opacity=0,
    postaction={
        draw=color2,
        opacity=1,
        decorate,
        decoration={parallel, raise=-0.75pt}
        },
    postaction={
        draw=color6,
        opacity=1,
        decorate,
        decoration={parallel, raise=0.75pt}
        }
    },
    color6color2ddntk2new/.style={
    dash pattern=on 1pt off 1pt,
    line width=1pt,
    draw=color6,
    opacity=0,
    postaction={
        draw=color6,
        opacity=1,
        decorate,
        decoration={parallel, raise=-0.75pt}
        },
    postaction={
        draw=color2,
        opacity=1,
        decorate,
        decoration={parallel, raise=0.75pt}
        }
    },
    color6color1color2ddntknew/.style={
    dash pattern=on 1pt off 1pt,
    line width=1pt,
    draw=color1,
    postaction={
        draw=color2,
        decorate,
        decoration={parallel, raise=-1.5pt}
        },
    postaction={
        draw=color6,
        decorate,
        decoration={parallel, raise=1.5pt}
        },
    },
    quarticblob/.style={
        /tikz/shape=circle,
        /tikz/draw=black,
        /tikz/fill=white!70!black,
        % tikzfeynman/particle={},
        /tikz/graphs/as={},
        /tikz/minimum size=15pt,
        % node contents={},
    },
    squareblob/.style={
        /tikz/shape=rectangle,
        /tikz/draw=black,
        /tikz/fill=white!70!black,
        % tikzfeynman/particle={},
        /tikz/graphs/as={},
        /tikz/minimum size=15pt,
        % node contents={},
    },
    smallblob/.style={
        /tikz/shape=circle,
        /tikz/draw=black,
        /tikz/fill=white!70!black,
        % tikzfeynman/particle={},
        /tikz/graphs/as={},
        /tikz/minimum size=6pt,
        /tikz/inner sep=0pt,
        % node contents={},
    },
    propblob/.style={
      /tikz/shape=circle,
      /tikz/draw=black,
      /tikz/fill=white,
      % tikzfeynman/particle={},
      /tikz/graphs/as={},
      /tikz/minimum size=15pt,
      % node contents={},
    },
    color6color1color2ddntk2new/.style={
    dash pattern=on 1pt off 1pt,
    line width=1pt,
    draw=color1,
    postaction={
        draw=color6,
        decorate,
        decoration={parallel, raise=-1.5pt}
        },
    postaction={
        draw=color2,
        decorate,
        decoration={parallel, raise=1.5pt}
        },
    },
    minidot/.style={
        /tikz/shape=circle,
        /tikz/draw=black,
        /tikz/fill=black,
        /tikz/graphs/as={},
        /tikz/inner sep=0pt,
        /tikz/outer sep=0pt,
        /tikz/minimum size=0.75mm,
    },
    meddot/.style={
        /tikz/shape=circle,
        /tikz/draw=black,
        /tikz/fill=gray,
        /tikz/graphs/as={},
        /tikz/inner sep=0pt,
        /tikz/outer sep=0pt,
        /tikz/minimum size=5mm,
    },
    color1doubghost/.style={
    transform canvas={shift={(0,-1pt)}},
    dash pattern=on 3pt off 3pt,
    line width=1pt,
    draw=color1,
    preaction={
      transform canvas={shift={(0,1pt)}},
      dash pattern=on 3pt off 3pt,
      line width=1pt,
      draw=color1
     }
    },
    color2doubghost/.style={
    transform canvas={shift={(0,-1pt)}},
    dash pattern=on 3pt off 3pt,
    line width=1pt,
    draw=color2,
    preaction={
      transform canvas={shift={(0,1pt)}},
      dash pattern=on 3pt off 3pt,
      line width=1pt,
      draw=color2
     }
    },
    doubghost/.style={
        dashed,
        double distance=1.5pt,
        thick,
    },
    color1blackghost/.style={
    transform canvas={shift={(0pt,-1pt)}},
    line width=1pt,
    preaction={
      transform canvas={shift={(0pt,1pt)}},
      dash pattern=on 3pt off 3pt,
      line width=1pt,
      draw=color1
    }
    },
    blackcolor1ghost/.style={
    transform canvas={shift={(0pt,-1pt)}},
    dash pattern=on 3pt off 3pt,
    line width=1pt,
    draw=color1,
    preaction={
      transform canvas={shift={(0pt,1pt)}},
      line width=1pt,
      draw=black
    }
    },
    color2blackghost/.style={
    transform canvas={shift={(0pt,-1pt)}},
    line width=1pt,
    preaction={
      transform canvas={shift={(0pt,1pt)}},
      dash pattern=on 3pt off 3pt,
      line width=1pt,
      draw=color2
    }
    },
    blackcolor2ghost/.style={
    transform canvas={shift={(0pt,-1pt)}},
    dash pattern=on 3pt off 3pt,
    line width=1pt,
    draw=color2,
    preaction={
      transform canvas={shift={(0pt,1pt)}},
      line width=1pt,
      draw=black
    }
    },
    color1color2dntknew/.style={
    dash pattern=on 1pt off 1pt,
    line width=1pt,
    draw=color6,
    opacity=0,
    postaction={
        draw=color1,
        opacity=1,
        decorate,
        decoration={parallel, raise=-0.75pt}
        },
    postaction={
        draw=color2,
        opacity=1,
        decorate,
        decoration={parallel, raise=0.75pt}
        }
    },
    color2color1dntknew/.style={
    dash pattern=on 1pt off 1pt,
    line width=1pt,
    draw=color6,
    opacity=0,
    postaction={
        draw=color2,
        opacity=1,
        decorate,
        decoration={parallel, raise=-0.75pt}
        },
    postaction={
        draw=color1,
        opacity=1,
        decorate,
        decoration={parallel, raise=0.75pt}
        }
    },
    color1color2blackghost/.style={
    transform canvas={shift={(0pt,-1pt)}},
    line width=1pt,
    draw=black,  
    preaction={
      transform canvas={shift={(0pt,1pt)}},
      dash pattern=on 3pt off 3pt,
      line width=1pt,
      draw=color2
      },
    preaction={
      transform canvas={shift={(0pt,2.5pt)}},
      dash pattern=on 3pt off 3pt,
      line width=1pt,
      draw=color1
      }  
    },
    blackcolor1color2ghost/.style={
    transform canvas={shift={(0pt,1pt)}},
    line width=1pt,
    draw=black,  
    preaction={
      transform canvas={shift={(0pt,-1pt)}},
      dash pattern=on 3pt off 3pt,
      line width=1pt,
      draw=color1
      },
    preaction={
      transform canvas={shift={(0pt,-2.5pt)}},
      dash pattern=on 3pt off 3pt,
      line width=1pt,
      draw=color2
      }  
    },
    ntkdntkcolor1color2/.style={
    transform canvas={shift={(0pt,1pt)}},
    dash pattern=on 3pt off 3pt,
    line width=1pt,
    draw=color1,
    preaction={
      transform canvas={shift={(0pt,-1pt)}},
      dash pattern=on 3pt off 3pt,
      line width=1pt,
      draw=color1
      },
    preaction={
      transform canvas={shift={(0pt,-2.5pt)}},
      dash pattern=on 3pt off 3pt,
      line width=1pt,
      draw=color2
      }  
    },
    color1color2ghost/.style={
    transform canvas={shift={(0,-1pt)}},
    dash pattern=on 3pt off 3pt,
    line width=1pt,
    draw=color2,
    preaction={
      transform canvas={shift={(0,1pt)}},
      dash pattern=on 3pt off 3pt,
      line width=1pt,
      draw=color1
     }
    },
    color2color1ghost/.style={
    transform canvas={shift={(0,-1pt)}},
    dash pattern=on 3pt off 3pt,
    line width=1pt,
    draw=color1,
    preaction={
      transform canvas={shift={(0,1pt)}},
      dash pattern=on 3pt off 3pt,
      line width=1pt,
      draw=color2
    }
    },
    color6color6color1color2ghost/.style={
    transform canvas={shift={(0pt,1pt)}},
    dash pattern =on 3pt off 3pt,
    line width=1pt,
    draw=color6,
    preaction={
      transform canvas={shift={(0pt,-1pt)}},
      dash pattern=on 3pt off 3pt,
      line width=1pt,
      draw=color6
      },
    preaction={
      transform canvas={shift={(0pt,-2.5pt)}},
      dash pattern=on 3pt off 3pt,
      line width=1pt,
      draw=color1
      },
    preaction={
      transform canvas={shift={(0pt,-4pt)}},
      dash pattern=on 3pt off 3pt,
      line width=1pt,
      draw=color2
      }
    },
    color6color1color2ddntk/.style={
    dash pattern=on 0.5pt off 1pt,
    line width=1pt,
    draw=color6,
    preaction={
      transform canvas={shift={(1pt,-1.5pt)}},
      dash pattern=on 0.5pt off 1pt,
      line width=1pt,
      draw=color1
     },
    preaction={
      transform canvas={shift={(2pt,-3pt)}},
      dash pattern=on 0.5pt off 1pt,
      line width=1pt,
      draw=color2
      }  
    },
    color6color1ddntk/.style={
    dash pattern=on 0.5pt off 1pt,
    line width=1pt,
    draw=color6,
      preaction={
      transform canvas={shift={(1pt,2pt)}},
      dash pattern=on 0.5pt off 1pt,
      line width=1pt,
      draw=color1
      }  
    },    
    color6color2ddntk/.style={
    dash pattern=on 0.5pt off 1pt,
    line width=1pt,
    draw=color6,
      preaction={
      transform canvas={shift={(1pt,-1.5pt)}},
      dash pattern=on 0.5pt off 1pt,
      line width=1pt,
      draw=color2
      }  
    },
    color6color1ddntk2/.style={
    dash pattern=on 0.5pt off 1pt,
    line width=1pt,
    draw=color1,
      preaction={
      transform canvas={shift={(0pt,2.5pt)}},
      dash pattern=on 0.5pt off 1pt,
      line width=1pt,
      draw=color6
      }  
    },
    color6color2ddntk2/.style={
    dash pattern=on 0.5pt off 1pt,
    line width=1pt,
    draw=color2,
      preaction={
      transform canvas={shift={(1pt,-1.5pt)}},
      dash pattern=on 0.5pt off 1pt,
      line width=1pt,
      draw=color6
      }  
    },
    ddntkddntkcolor1color2ghost/.style={
    transform canvas={shift={(0pt,1.5pt)}},
    dash pattern=on 3pt off 3pt,
    line width=1pt,
    draw=color6,
    preaction={
      transform canvas={shift={(0pt,3pt)}},
      dash pattern=on 3pt off 3pt,
      line width=1pt,
      draw=color1
      },
    preaction={
      transform canvas={shift={(0pt,-1.5pt)}},
      dash pattern=on 3pt off 3pt,
      line width=1pt,
      draw=color6
      },
    preaction={
      transform canvas={shift={(0pt,-3pt)}},
      dash pattern=on 3pt off 3pt,
      line width=1pt,
      draw=color2
      }  
    },
    color6blackghost/.style={
    transform canvas={shift={(0pt,-1pt)}},
    line width=1pt,
    preaction={
      transform canvas={shift={(0pt,1pt)}},
      dash pattern=on 3pt off 3pt,
      line width=1pt,
      draw=color6
    }
    },
    blackcolor6ghost/.style={
    transform canvas={shift={(0pt,-1pt)}},
    dash pattern=on 3pt off 3pt,
    line width=1pt,
    draw=color6,
    preaction={
      transform canvas={shift={(0pt,1pt)}},
      line width=1pt,
      draw=black
    }
    },
    ntkdntkcolor2color2color6/.style={
    transform canvas={shift={(0pt,1pt)}},
    dash pattern=on 3pt off 3pt,
    line width=1pt,
    draw=color2,
    preaction={
      transform canvas={shift={(0pt,-1pt)}},
      dash pattern=on 3pt off 3pt,
      line width=1pt,
      draw=color2
      },
    preaction={
      transform canvas={shift={(0pt,-2.5pt)}},
      dash pattern=on 3pt off 3pt,
      line width=1pt,
      draw=color6
      }  
    },
    ntkdntkcolor6color1color1/.style={
    transform canvas={shift={(0pt,2.5pt)}},
    dash pattern=on 3pt off 3pt,
    line width=1pt,
    draw=color6,
    preaction={
      transform canvas={shift={(0pt,1pt)}},
      dash pattern=on 3pt off 3pt,
      line width=1pt,
      draw=color1
      },
    preaction={
      transform canvas={shift={(0pt,-1pt)}},
      dash pattern=on 3pt off 3pt,
      line width=1pt,
      draw=color1
      }  
    },
    ntkdntkcolor1color2color6/.style={
    transform canvas={shift={(0pt,1pt)}},
    dash pattern=on 3pt off 3pt,
    line width=1pt,
    draw=color1,
    preaction={
      transform canvas={shift={(0pt,-1pt)}},
      dash pattern=on 3pt off 3pt,
      line width=1pt,
      draw=color2
      },
    preaction={
      transform canvas={shift={(0pt,-2.5pt)}},
      dash pattern=on 3pt off 3pt,
      line width=1pt,
      draw=color6
      }  
    },
    ntkdntkblackcolor1color2color6/.style={
    transform canvas={shift={(0pt,1pt)}},
    dash pattern=on 3pt off 3pt,
    line width=1pt,
    draw=color1,
    preaction={
      transform canvas={shift={(0pt,2.5pt)}},
      line width=1pt,
      draw=black
      },
    preaction={
      transform canvas={shift={(0pt,-1pt)}},
      dash pattern=on 3pt off 3pt,
      line width=1pt,
      draw=color2
      },
    preaction={
      transform canvas={shift={(0pt,-2.5pt)}},
      dash pattern=on 3pt off 3pt,
      line width=1pt,
      draw=color6
      }  
    },
     ntkdntkcolor6color1color2/.style={
    transform canvas={shift={(0pt,2.5pt)}},
    dash pattern=on 3pt off 3pt,
    line width=1pt,
    draw=color6,
    preaction={
      transform canvas={shift={(0pt,1pt)}},
      dash pattern=on 3pt off 3pt,
      line width=1pt,
      draw=color1
      },
    preaction={
      transform canvas={shift={(0pt,-1pt)}},
      dash pattern=on 3pt off 3pt,
      line width=1pt,
      draw=color2
      }  
    },
    ntkdntkcolor6color1color2black/.style={
    transform canvas={shift={(0pt,2.5pt)}},
    dash pattern=on 3pt off 3pt,
    line width=1pt,
    draw=color6,
    preaction={
      transform canvas={shift={(0pt,1pt)}},
      dash pattern=on 3pt off 3pt,
      line width=1pt,
      draw=color1
      },
    preaction={
      transform canvas={shift={(0pt,-1pt)}},
      dash pattern=on 3pt off 3pt,
      line width=1pt,
      draw=color2
      },
    preaction={
      transform canvas={shift={(0pt,-2.5pt)}},
      line width=1pt,
      draw=black
      }
    }
}

%%% Local Variables:
%%% mode: LaTeX
%%% TeX-master: "ntk_feynman"
%%% End:

